The Power of the Weak

A landmark result in the study of logics for formal verification is Janin & Walukiewicz's theorem, stating that the modal $\mu$-calculus ($\mu\mathrm{ML}$) is equivalent modulo bisimilarity to standard monadic second-order logic (here abbreviated as $\mathrm{smso}$), over the class of labelled transition systems (LTSs for short). Our work proves two results of the same kind, one for the alternation-free fragment of $\mu\mathrm{ML}$ ($\mu_D\mathrm{ML}$) and one for weak $\mathrm{mso}$ ($\mathrm{wmso}$). Whereas it was known that $\mu_D\mathrm{ML}$ and $\mathrm{wmso}$ are equivalent modulo bisimilarity on binary trees, our analysis shows that the picture radically changes once we reason over arbitrary LTSs. The first theorem that we prove is that, over LTSs, $\mu_D\mathrm{ML}$ is equivalent modulo bisimilarity to noetherian $\mathrm{mso}$ ($\mathrm{nmso}$), a newly introduced variant of $\mathrm{smso}$ where second-order quantification ranges over "well-founded" subsets only. Our second theorem starts from $\mathrm{wmso}$, and proves it equivalent modulo bisimilarity to a fragment of $\mu_D\mathrm{ML}$ defined by a notion of continuity. Analogously to Janin & Walukiewicz's result, our proofs are automata-theoretic in nature: as another contribution, we introduce classes of parity automata characterising the expressiveness of $\mathrm{wmso}$ and $\mathrm{nmso}$ (on tree models) and of $\mu_C\mathrm{ML}$ and $\mu_D\mathrm{ML}$ (for all transition systems).

==> ale/20181407-ssec-fixnoet.tex <==
\subsection{Fixpoints of noetherian maps}

We will now see how to prove Proposition~\ref{p:keyfix}(1), which is the key 
result that we need to embed alternation-free $\mu$-calculi such as 
$\mu_{D}\ofoe$ and $\mu_{D}\ML$ into noetherian second-order logic.
Perhaps suprisingly, this case is slightly more subtle than the characterisation of
fixpoints of continuous maps.

We start with stating some auxiliary definitions and results on monotone 
functionals, starting with a game-theoretic characterisation of their least
fixpoints~\cite{Ven08}.

\begin{definition}
\label{d:unfgame}
Given a monotone functional $F: \pow(S)\to \pow(S)$ we define the 
\emph{unfolding game} $\UG_{F}$ as follows:
\begin{itemize}
\item at any position $s \in S$, $\eloise$ needs to pick a set $X$ such that 
$s \in FX$;
\item at any position $X \in \pow(S)$, $\abelard$ needs to pick an element of 
$X$
\item all infinite matches are won by $\abelard$.
\end{itemize}
A positional strategy $\ystrat: S \to \pow(S)$ for $\eloise$ in $\UG_{F}$ is 
\emph{descending} if, for all ordinals $\alpha$,
\begin{equation}
\label{eq:dec}
s \in F^{\alpha+1}(\nada) \text{ implies } \ystrat(s) \sse F^{\alpha}(\nada).
\end{equation}
\end{definition}

It is not the case that \emph{all} positional winning strategies for $\eloise$ 
in $\UG_{F}$ are descending, but the next result shows that there always is one.

\begin{proposition}
\label{p:unfg}
The following hold for any monotone functional $F: \pow(S)\to \pow(S)$:
\begin{enumerate}[(1)]
\item
for all $s \in S$, $s \in \win_{\eloise}(\UG_{F})$ iff $s \in \LFP. F$;
\item if $s \in \LFP. F$, then \eloise has a descending winning strategy in 
$\UG_{F}@s$.
\end{enumerate}
\end{proposition}

\begin{proof}
Point (1) corresponds to \cite[Theorem 3.14(2)]{Ven08}.
For part (2) one can simply take the following strategy.
Given $s \in \LFP.F$, let $\alpha$ be the least ordinal such that $s \in 
F^{\alpha}(\nada)$; it is easy to see that $\alpha$ must be a successor ordinal,
say $\alpha = \beta + 1$. 
Now simply put $\ystrat(s) := F^{\beta}(\nada)$.
\end{proof}

\begin{definition}
\label{d:str-tree}
Let $F: \pow(S)\to \pow(S)$ be a monotone functional, let $\ystrat$ be a 
positional winning strategy for $\eloise$ in $\UG_{F}$, and let $r \in S$. 
Define $T_{\ystrat,r} \sse S$ to be the set of states in $S$ that are 
$\ystrat$-reachable in $\UG_{F}@r$.
This set has a tree structure induced by the map $\ystrat$ itself, where the 
children of $s \in T_{\ystrat,r}$ are given by the set $\ystrat(s)$; we will
refer to $T_{\ystrat,r}$ as the \emph{strategy tree} of
$\ystrat$.
\end{definition}
Note that a strategy tree $T_{\ystrat,r}$ will have no infinite paths, since we
define the notion only for a \emph{winning} strategy $\ystrat$.

\begin{proposition}
\label{p:afmc-2}
Let $F: \pow(S)\to \pow(S)$ be a monotone functional, let $r \in S$, and let 
$\ystrat$ be a descending winning strategy for $\eloise$ in $\UG_{F}$.
Then
\begin{equation}
\label{eq:afmc3}
r \in \LFP. F \text{ implies } r \in \LFP. F\rst{T_{\ystrat,r}}.
\end{equation}
\end{proposition}

\begin{proof}
Let $F,r$ and $\ystrat$ be as in the formulation of the proposition.
% The direction from right to left in \eqref{eq:afmc3} is immediate by
% Proposition~\ref{p:rstfix}.
% For the opposite direction, 
Assume that $r \in \LFP. F$, then clearly $r \in F^{\al}(\nada)$ for some 
ordinal $\al$; furthermore, $T_{\ystrat,r}$ is defined and clearly we have 
$r \in T_{\ystrat,r}$.
Abbreviate $T \isdef T_{\ystrat,r}$
It then clearly suffices to show that for all ordinals $\alpha$ we have
\begin{equation}
\label{eq:unf1}
F^{\al}(\nada) \cap T \sse (F\rst{T})^{\alpha}(\nada).
\end{equation}
We will prove \eqref{eq:unf1} by transfinite induction.
The base case, where $\alpha = 0$, and the inductive case where $\alpha$ is a 
limit ordinal are straightforward, so we focus on the case where $\alpha$ is a 
successor ordinal, say $\alpha = \beta +1$.
Take an arbitrary state $u \in F^{\beta+1}(\nada) \cap T$, then we 
find $\ystrat(u) \sse F^{\beta}(\nada)$ by our assumption \eqref{eq:dec}, and 
$\ystrat(u) \sse T$ by definition of $T$.
Then the induction hypothesis yields that 
$\ystrat(u) \sse (F\rst{T})^{\beta}(\nada)$, and so we have 
$\ystrat(u) \sse (F\rst{T})^{\beta}(\nada) \cap T$.
But since $\ystrat$ is a winning strategy, and $u$ is a winning position for 
$\eloise$ in $\UG_{F}$ by Claim~\ref{p:unfg}(i), $\ystrat(u)$ is a
legitimate move for $\eloise$, and so we have $u \in F(\ystrat(u))$.
Thus by monotonicity of $F$ we obtain $u \in 
F((F\rst{T})^{\beta}(\nada) \cap T)$, and since $u \in T$ 
by assumption, this means that $u \in (F\rst{T})^{\beta+1}(\nada)$ as 
required.
\end{proof}

We now turn to the specific case where we consider the least fixed point of a 
functional $F$ which is induced by some formula $\phi(p) \in 
\mu_{D}\mathcal{L}_1$ on some LTS $\bbS$.   
By Proposition \ref{p:unfg} and Fact~\ref{f:adeqmu}, we have that $\eloise$ has
a winning strategy in  $\egame(\mu p.\phi(p),\bbS)@(\mu p.\phi(p),s)$ if and only if she has one in $\UG_{F}@s$ too, where $F := \phi_{p}^{\bbS}$ is the monotone functional defined by $\phi(p)$. The next Proposition  makes this correspondence explicit when $\mathcal{L}_1=\foe$. 

First, we need to introduce some auxiliary concepts and notations.
Given  a winning strategy   $\ystrat$ for $\eloise$ in $\egame(\mu p. \phi,\bbS)@(\mu p. \phi,s)$, 
let $B(\ystrat)$ be the set of all finite $\ystrat$-guided, possibly partial, 
matches in  $\egame(\psi,\bbS)@(\psi,s)$ in which no position of the form 
$(\nu q. \psi, r)$ is visited. 
$\eloise$ is said to have \emph{compatible} positional winning strategies
$\chi$ in $\UG_F@s$ and  $\chi'$  in $\egame(\mu p.\phi,\bbS)@(\mu p.\phi,s)$ if
each point in $T_{\chi,s}$ lies on some path belonging to $B^\bbS(\chi')$. 

\btbs
\item
please define $B^\bbS(\chi')$
\etbs

\begin{proposition}\label{p:unfold=evalgame2}
%Player $\exists$ has a winning strategy $\chi$ in $\UG_F@(s,\phi(p))$ if and only she has winning strategy $\chi'$ in 
%$\egame(\mu p.\phi,\bbS)@(s, \mu p.\phi)$. 
%Moreover it holds that each $r \in  T_{\chi,s}$ lies in some path in $B^\bbS(\chi')$.
%$s \in \ext{\mu p.\phi(p)}^{\bbS}$, with 
The following hold, for any formula $\phi(p) \in \mu_{D}\foe{p}$:
\begin{enumerate}[(1)]
\item For every positional winning strategy $\chi$ for $\eloise$ in $\UG_F@s$,
there is a compatible positional winning strategy $\chi'$ for her in 
$\egame(\mu p.\phi,\bbS)@(\mu p.\phi,s)$;
\item For every positional winning strategy $\chi'$ for $\eloise$ in 
$\egame(\mu p.\phi,\bbS)@(\mu p.\phi,s)$, there is a compatible  positional 
winning strategy $\chi$ for her in $\UG_F@s$.
\end{enumerate}
\end{proposition}

\begin{proof}
For the first statement of the Proposition we reason as follows. 
Let $\chi: S \to \pow{(S)}$  be a positional winning strategy for $\eloise$ in $\UG_F@s$. 
Hence, for every $t \in \win_{\eloise}(\UG_{F})$, it holds that $t \in F(\chi(t))$ 
and therefore that there is a positional winning strategy $\chi_t$ for $\eloise$ 
in the game $\egame(\phi,\bbS[p \mapsto \chi(s)])$ starting at $(\phi,t)$. 
%\btbs
%\item
%YV: I get confused with the T,t and $\chi, s$.
%\etbs
Let $\chi'$ be the following strategy for $\eloise$ in
$\egame(\mu p.\phi,\bbS)@(\mu p.\phi,s)$:
\begin{enumerate}
\item after the initial automatic move, the position of the match is $(\phi,s)$; 
$\eloise$ first plays her strategy $\chi_s$;
\item each time a position $(p,t)$ is reached, 
\begin{enumerate}
%necessarily 
\item if $t \in \win_{\eloise}(\UG_{F})$, then $\eloise$ continues with $\chi_t$;
\item if $t \notin \win_{\eloise}(\UG_{F})$, then $\eloise$ continues with a random positional strategy.
\end{enumerate}
\end{enumerate}
We verify that this positional strategy is actually a compatible positional 
winning strategy for her.

\btbs
\item
Why is $\chi'$ positional?
Do we actually need the strategy to be positional?
\etbs

First of all, observe that every position of the form $(p,t)$ reached during
a $\chi'$-guided match, we have $t \in \win_{\eloise}(\UG_{F})$. 
This can be proved by induction on the number of position of the form $(p,t)$
visited during a $\chi'$-guided match. 
For the inductive step, assume $w \in \win_{\eloise}(\UG_{F})$. 
Hence $\chi_w$ is winning for $\eloise$ in  $\egame(\phi,\bbS[p \mapsto 
  \chi(w)])@(\phi,w)$. 
This means that if a position of the form $(p, t)$ is reached, the variable $p$ 
must be true at $t$ in the model $\bbS[p \mapsto \chi(w)]$, meaning that it
belongs to the set $\chi(w)$.
By assumption $\chi$ is a winning strategy for $\eloise$ in $\UG_F$, and 
therefore any element of $\chi(w)$ is again a member of the set 
$\win_{\eloise}(\UG_{F})$. 

Finally, let $\pi$ be an arbitrary $\chi'$-guided match of $\egame(\phi,
\bbS[p \mapsto \chi(w)])@(\phi,w)$. 
We verify that $\pi$ is winning for $\eloise$. 
First observe that since $\chi$ is winning for her in $\UG_F@s$, the fixpoint 
variable $p$ is unfolded only finitely many times during $\pi$. 
Let $(p,t)$ be the last basic position in $\pi$ where $p$ occurs. 
Then from now on $\chi'$ and $\chi_t$ coincide, yielding  that the match is 
winning for $\eloise$. Clearly $\chi'$ and $\chi$ are compatible.

\btbs
\item
Why is that so clear?
\etbs

\newpage

Now we turn to part (2) of the Proposition.
Let $\chi'$ be a positional winning strategy for $\eloise$ in 
$\egame(\mu p.\phi(p),\bbS)@(\mu p.\phi(p),s)$. 
Let $B(\chi')$ be the set of all finite $\chi'$-guided partial matches in 
$\egame$, 

\btbs
\item
If $B(\chi')$ is indeed different from the earlier defined $B(\chi')$, 
better give it a different name.
\etbs

let $\pi\in B(\chi')$ and define \[P_{\last(\pi)}:=\{ (p,w) \mid \exists \pi' \in B(\chi'), \pi'=\pi \rho(p,w), p\text{ does not occur in }\rho\}.\]

It is not hard to derive from the positionality of $\chi'$ that for every $\pi, 
\pi' \in B(\chi')$ such that $\last(\pi)=\last(\pi')$, it holds that $\pi\rho 
\in B(\chi')$ if and only if $\pi'\rho \in B(\chi')$, for every finite match 
$\rho$.

Now consider  the positional strategy $\ystrat$ in $\UG_{F}@s$ defined by 
\[
\chi(t) \isdef \{ w \mid (p,w) \in P_{\last(\pi)}, \pi\in B(\chi'), 
\last(\pi)=(\mu p. \phi(p), t)\}.
\]
\btbs
\item
?? We can only have $\last(\pi)=(\mu p. \phi(p), t)$ if $\pi$ is a trivial
match of lenght 1
\item
Why is $\chi$ positional?
\etbs

%While playing the unfolding game $\UG$, $\eloise$ builds an 
%$\chi'$-guided `shadow match' $\egame(\mu p.\phi(p),\bbS)@(\mu p.\phi(p),s)$ 
%such that the positions in the $\UG$-match of the form $t$ exactly correspond to
%the positions of the form $(\phi(p),t)$ in the evaluation game $\egame$.

Compatibility being immediate, it suffices to verify that $\ystrat$ is winning for $\eloise$. First of all, since $\chi'$ is winning, $B(\chi')$ does not contain an infinite 
ascending chain of $\chi'$-guided matches, and thence any  $\chi$-guided match in $\UG_{F}@s$ is finite. It therefore remains to verify that for every $\chi$-guided match $\pi$ in $\UG_{F}@s$ such that $\last(\pi)$ is an $\eloise$ position, she can always move. But this is immediate since 
\begin{itemize}
\item $(\mu p. \phi(p), s) \in \last(B(\chi'))$, 
\item if $(\mu p. \phi(p), t) \in \last(B(\chi'))$, then %$(\phi(p), t) \in \last(B(\chi'))$ and  
$\chi'$ is (naturally induces) a winning strategy for $\eloise$ in $\egame(\phi(p),\bbS[p \mapsto \chi(t)])@(\phi(p),t)$, and thus in particular $t \in F(\chi(t))$,
\item if $(p, t) \in \last(B(\chi'))$ then $(\mu p. \phi(p), t) \in \last(B(\chi'))$,
\end{itemize}
%\btbs
%\item YV: some more detail here?
%\etbs
where $\last(B(\chi')):=\{\last(\pi) \mid \pi \in B(\chi')\} \subseteq \win_{\eloise}(\egame(\mu p.\phi(p),\bbS))$.
\end{proof}

%Notice that the evaluation game for the modal $\mu$ calculus can be easily adapted to $\mu_{D}\foe$ and provide a corresponding Adequacy Theorem (Proposition \ref{p:unfold=evalgame}). In particular, we would have that 
%$\eloise$ has a winning strategy in  $\egame(\mu p.\phi(p),\bbS)@(\mu p.\phi(p),s)$ if and only if $s \in \ext{\mu p.\phi(p)}^{\bbS}$, with $\phi(p) \in \mu_{D}\foe{p}$.

\begin{proofof}{Proposition~\ref{p:keyfix}(1)}
%    
%\btbs
%\item
%the argument below needs to be thoroughly checked.
%\etbs
Let $\bbS$ be an LTS and $\phi(p) \in \mu_{D}\ofoe{p}$. 

The right-to-left direction of \eqref{eq:foe-d} being proved by 
Proposition \ref{p:rstfix}, we check the left-to-right direction.
We first verify that winning strategies in evaluation games for noetherian 
fixpoint formulas naturally induce bundles. 
More precisely:
\medskip
%Given  a winning strategy   $\ystrat$ for $\eloise$ in $\egame(\mu p. \phi,\bbS)@(\mu p. \phi,s)$,  let $B(\ystrat)$ be the set of all finite $\ystrat$-guided, possibly partial, matches in  $\egame(\psi,\bbS)@(\psi,s)$ in which a position of the form $(\nu q. \psi, r)$ is not visited.

\textsc{Claim}
% \begin{claim*}\label{p:strategybundledEv}
Let $B^\bbS(\ystrat)$ be the projection of $B(\ystrat)$ on $S$, that is the set
of all paths in $\bbS$ that are a projection on $S$ of a $\ystrat$-guided 
(partial) match in $B(\ystrat)$. Then $B^\bbS(\ystrat)$ is a bundle.
% \end{claim*}
\medskip

\begin{pfclaim}
Assume towards a contradiction that $B^\bbS(\ystrat)$ contains an infinite 
ascending chain $\pi_{0} \sqsubset \pi_{1} \sqsubset \cdots$. 
Let $\pi$ be its limit and consider the set of elements in $B(\ystrat)$ that,
projected on $S$, are prefixes of $\pi$. 
By  K\"{o}nig's Lemma, this set contains an infinite ascending chain whose 
limit is an infinite $\ystrat$-guided match in $\egame(\mu p. \phi,\bbS)$
which starts at $(\mu p. \phi,s)$, and of which $\pi$ is the projection on $S$.
By definition of $B(\ystrat)$,  the highest bound variable of $\mu p. \phi$ 
that gets unravelled infinitely often in $\rho$ is a $\mu$-variable, meaning 
that the match is winning for $\abelard$, a contradiction.
\end{pfclaim}

Then, let $F := \phi_{p}^{\bbS}$ be the monotone functional defined by $\phi(p)$.
Assume that $s \in \ext{\mu p.\phi}^{\bbS}$. 
This means that $s \in \LFP. F$, and by Proposition~\ref{p:afmc-2}, we obtain 
that $s \in \LFP. F\rst{T_{\ystrat,r}}$.
We verify that $T_{\chi, s}$ is noetherian.
Applying Proposition~\ref{p:unfg} to the fact that $s \in \LFP. F$ yields that 
$\eloise$ has a descending winning strategy $\chi$ in $\UG_{F}@s$. 
By Proposition \ref{p:unfold=evalgame2}, $\eloise$ has a winning strategy 
$\chi'$ in $\egame(\mu p.\phi,\bbS)@(\mu p.\phi,s)$ compatible with $\chi$.
Because of compatibility, every node in $T_{\chi, s}$ lies on some path of 
$B^\bbS(\ystrat)$. 
From the Claim
% Claim \ref{p:strategybundledEv}
we known that $B^\bbS(\ystrat)$ is a bundle, meaning that  $T_{\chi, s}$ is
noetherian as required.   
\end{proofof}


==> commands.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%NEXT


% claims
\makeatletter
\newcounter{ourclaimcounter}
\newenvironment{ourclaim}{%
 	\stepcounter{ourclaimcounter}%
	\def\@currentlabel{\theourclaimcounter}%
	\begin{trivlist}\item[]{\sc Claim~\arabic{ourclaimcounter}.~}
	}
	{\end{trivlist}
        }
\newenvironment{claimfirst}{%
	\setcounter{ourclaimcounter}{0}%
	\begin{ourclaim}}{\end{ourclaim}}
\makeatother

% to be supplied
\newenvironment{tbs}{%
   \small\tt
   \begin{enumerate}[$\blacktriangleright$]}{\end{enumerate}}
\newcommand{\btbs}{\begin{tbs}}
\newcommand{\etbs}{\end{tbs}}
\newcommand{\shtbs}[1]{\begin{tbs} \item #1 \end{tbs}}

\newcommand{\todo}{\marginpar{$\bullet$}}

%%%%%%%%%% LEFTOVERS %%%%%%%%

%\newcommand*\sepsection{\bigskip}

% \newcommand{\umods}{\mathfrak{M}_1}
% \newcommand{\sumods}{\umods^s}
% \newcommand{\rest}{|}
% \newcommand{\iso}{\simeq}
% \newcommand{\resto}{{\upharpoonright}}
% \newcommand{\dcup}{\uplus}
% \newcommand{\stl}{\rightarrowtriangle} %\prec}
% \newcommand{\tc}{\mathsf{TC}}
% \newcommand{\st}{\mathrm{ST}}
% \newcommand{\ot}{\mathrm{OT}}
% \newcommand{\sorts}{\mathcal{S}}
% \newcommand{\asort}{\mathtt{s}}
% \newcommand{\aSort}{\mathtt{S}}
% \newcommand{\pto}{\rightharpoonup}
% \newcommand{\llet}{\subseteq}
% \newcommand{\lletneq}{\subsetneq}
% \newcommand{\ffunc}[2]{F^{#1}_{#2}}
% \newcommand{\somemod}{\heartsuit}
% \newcommand{\gsubmodel}[2]{{#1}^{\downarrow}_{#2}}
% \newcommand{\gsubaut}[2]{{#1}^{\blacktriangle}_{#2}}
% \newcommand{\pleadsto}[1]{R^{\shortrightarrow}_{#1}}

% \newcommand{\omls}{\oml^\flat}
% \newcommand{\oca}{\ensuremath{\mathrm{ADD}_1}\xspace}
% \newcommand{\ocm}{\ensuremath{\mathrm{MUL}_1}\xspace}
% \newcommand{\ocam}{\ensuremath{\oca^s}\xspace}
% \newcommand{\ocmm}{\ensuremath{\ocm^s}\xspace}
% \newcommand{\ogcam}{\ensuremath{\textup{g}\oca^s}\xspace}
% \newcommand{\ogcmm}{\ensuremath{\textup{g}\ocm^s}\xspace}

% mu-calculi
% \newcommand{\mucaML}{\ensuremath{\mu_{a}\ML}\xspace}
% \newcommand{\nmucaML}{\ensuremath{\mu_{na}\ML}\xspace}
% \newcommand{\rmucaML}{\ensuremath{\mu_{a}^{-}\ML}\xspace}
% \newcommand{\rnmucaML}{\ensuremath{\mu_{na}^{-}\ML}\xspace}
% \newcommand{\lmuML}{\ensuremath{\mu\ML^{\lor}}\xspace}
% \newcommand{\lmucML}{\ensuremath{\mu_{C}\ML^{\lor}}\xspace}
% \newcommand{\lnmucML}{\ensuremath{\mu_{nc}\ML^{\lor}}\xspace}
% \newcommand{\mufoe}{\ensuremath{\mu\foe}\xspace}
% \newcommand{\mufoei}{\ensuremath{\mufoe^\infty}\xspace}
% \newcommand{\mucfoe}{\ensuremath{\mu_{c}\foe}\xspace}
% \newcommand{\mucfoei}{\ensuremath{\mu_{c}\foe^\infty}\xspace}
% \newcommand{\mucafoe}{\ensuremath{\mu_{a}\foe}\xspace}
% \newcommand{\so}[1]{\mathrm{SO}(#1)}
% \newcommand{\afmc}{\ensuremath{\mathrm{AFMC}}\xspace}
% \newcommand{\muMC}{\ensuremath{\Sigma\mu\ML}}    %least fixpoint-fragment of Mu-calculus
% \newcommand{\muffoe}{\ensuremath{\mufoe^\ff}\xspace}
% \newcommand{\muffoei}{\ensuremath{{\mufoei}^\ff}\xspace}
% \newcommand{\mucaffoe}{\ensuremath{\mucafoe^\ff}\xspace}
% \newcommand{\mucffoei}{\ensuremath{{\mucfoei}^\ff}\xspace}

% \newcommand{\matches}{\mathcal{B}}
% \newcommand{\match}{\pi}
% \newcommand{\fwa}[2]{{#1}^{\!\div}_{#2}} %{\mathsf{\fconst}^{#2}_{wa}(#1)}
% \newcommand{\fwc}[2]{{#1}^{\!\div}_{#2}} %{\mathsf{\fconst}^{#2}_{wa}(#1)}

% \newcommand{\sgame}{\mathcal{S}}
% \newcommand{\agamesym}{\mathcal{A}_\textrm{s}}
% \newcommand{\agamenfa}{\underline{\mathcal{A}}} %{\mathcal{A}_\textrm{FA}}
% \newcommand{\xgame}{\mathcal{X}}

% \newcommand{\aut}{\ensuremath\mathbb{A}\xspace}
% \newcommand{\baut}{\ensuremath\mathbb{B}\xspace}
% \newcommand{\iaut}{\ensuremath\mathbb{X}\xspace}
% \newcommand{\efgame}{\mathrm{EF}}
% \newcommand{\game}{\mathcal{G}}

% \newcommand{\toprops}[1]{\varpi_c}
% \newcommand{\compset}[1]{\{#1\}}



==> fabio/stuff-on-functionality.tex <==
\section{Text on functionality}

\bigskip\hrule\bigskip
THIS TEXT TO BE MOVED TO AUTOMATA PAPER
\bigskip\hrule\bigskip

\begin{definition}
An $A$-valuation $V: A \to \wp D$ is said to \emph{separate} a set $B
\subseteq 
A$ if $\sz{V^{\flat}(d) \cap B} \leq 1$, for every $d \in D$.
%
A sentence $\phi \in \ofoei(A)$ is \emph{$B$-separating}
% , for a subset $B \subseteq A$,
if for every valuation $V: A \to \wp D$ such that $(D,V) \models 
\phi$ there is a $B$-separating valuation $U \leq_{B} V$ such that
$(D,U) 
\models \phi$.
\end{definition}

Intuitively, a formula $\phi$ is $B$-separating if its truth in a
monadic model 
never requires an element of the domain to satisfy two distinct
predicates in 
$B$ at the same time, in the sense that any valuation violating this
constraint
can be reduced to a valuation satisfying it, without sacrificing the
truth of
$\phi$.

\begin{lemma}
With $B \subseteq A$, let $\phi \in (\ofoei)^{+}(A)$ be a disjunction 
of formulas of the shape
$\mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{\Sigma}{+}$, where
$\Sigma\subseteq \pw A$, $\Psi, \vlist{T} \subseteq \pw B$ are such
that
(1) $B \cap \bigcup\Sigma = \nada$ and 
(2) each $S \in \vlist{T} \cup \Psi$ is either empty or a singleton
from $B$. 
Then $\phi$ is both separating and continuous in $B$.
\end{lemma}

As a consequence, under the same conditions as in the lemma, for
every valuation
$V: A \to \wp D$ such that $(D,V) \models \phi$ we may find a
$B$-separating 
valuation $U$ such that $(D,U) \models \phi$ and
(1) $U(b)$ is a finite subset of $V(b)$, for all $b \in B$, and
(2) $U(a) = V(a)$, for all $a \in A \setminus B$.

\bigskip\hrule\bigskip

\newpage


\bigskip\hrule\bigskip

THE FOLLOWING IS LEFT OVER FROM THE SECTION ON MONOTONICITY

\bigskip\hrule\bigskip

We isolate the case when basic forms enforce a semantic property
called 
\emph{functionality}. 
This will be useful when defining non-deterministic parity automata.

\begin{definition}\label{def:functionalsentenceofoe}
We say that $\varphi \in \ofoe(A)$ is \emph{functional} in
$B\subseteq A$ if 
whenever $(D,V \: A \to \wp(D)) \models \varphi$ then there is a
restriction 
$V'$ of $V$ such that $(D,V' \: A \to \wp(D)) \models \varphi$ and $s
\in V'(b)$
for $b \in B$ implies $s \not\in V'(a)$ for all $a \in
A\setminus\{b\}$.
\end{definition}

The syntactic shape guaranteeing functionality is the following.
\begin{proposition}\label{lemma:functionalsentenceofoe} 
Suppose that $\varphi \in \ofoe(A)$ is equivalent to a sentence in
the basic form
$\bigvee \posdbnfofoe{\vlist{T}}{\Pi}$ where $T_1, \dots, T_k$ and
each $S \in 
\Pi$ are either $\emptyset$ of singletons $\{b\}$ for some $b \in B$. 
\todo % reformulate
Then $\varphi$ is functional in $B$.
\end{proposition}

\begin{proof} 
Let $(D,V)$ be a model where $\varphi$ is true. Thus one disjunct
$\posdbnfofoe{\vlist{T}}{\Pi}$ is true, that means, there are
elements $s_1, \dots, s_k$ of $D$ witnessing types $T_1, \dots, T_k$
respectively and all the other elements witness some $S \in \Pi$. By
pruning from $V$ any other assignment of predicates to elements of
$D$ but for the types they witness according to this description, we
obtain a restriction $V'$ of $V$ such that $(D,V) \models \varphi$.
Because $T_1, \dots, T_k$ are either $\emptyset$ of singletons
$\{b\}$ for some $b \in B$, such $V'$ assigns at most one $b \in B$
to each element of $D$. Therefore $\varphi$ is functional in $B$.
\end{proof}
\bigskip\hrule\bigskip

As for $\ofoe$, we record a syntactic criterion for functionality,
which is
defined as in Definition \ref{def:functionalsentenceofoe} with
$\ofoei$ 
replacing $\ofoe$. 

\begin{definition}We say that $\varphi \in \ofoe(A)$ is
\emph{functionally continuous} in $B\subseteq A$ if whenever $(D,V \:
A \to \wp(D)) \models \varphi$ then there is a restriction $V'$ of
$V$ such that $(D,V' \: A \to \wp(D)) \models \varphi$ and for all $b
\in B$
\begin{description}
\item[functionality] $s \in V'(b)$ implies $s \not\in V'(a)$ for all
$a \in A\setminus\{b\}$
\item[continuity] $V'(b)$ is finite.
\end{description}
\end{definition}

\begin{proposition}\label{lemma:functionalsentenceofoe} 
If $\varphi \in \ofoe(A)$ is in the basic form $\bigvee 
\posdbnfofoei{\vlist{T}}{\Pi}{\Sigma}$ with all $T_1, \dots, T_k,\Pi$
either 
empty or singletons, then it is functional in $A$.
\end{proposition}

\newpage

\bigskip\hrule\bigskip

THE FOLLOWING IS LEFT OVER FROM THE SECTION ON CONTINUITY

\bigskip\hrule\bigskip

Putting together the above lemmas we obtain
Theorem~\ref{thm:ofoeicont}.
Moreover, a careful analysis of the translation gives us the
following corollary, 
providing normal forms for the continuous fragment of $\ofoei$. 
Point \ref{pt:ofoeifunctionalcontinuous} below is tailored for
applications to
parity automata, see Theorem~\ref{PROP_facts_finConstrwmso}. 
We call a formula $\phi  \in \ofoei(A)$ \emph{functionally
continuous} in
$B \subseteq A$ when, given a model $(D,V),g$ where $\phi$ is true, a 
restriction $V'$ of $V$ can be found that both witnesses continuity
in each
$b \in B$ and also witnesses functionality in each $b \in B$, in the
sense of
Definition \ref{def:functionalsentenceofoe}.

\begin{corollary}\label{cor:ofoeicontinuousnf}
Let $\phi \in \ofoei(A)$, the following hold:
\begin{enumerate}[(i)]
\item 
The formula $\phi$ is continuous in $a \in A$ iff it is equivalent to
a 
formula in the basic form $\bigvee
\mondbnfofoei{\vlist{T}}{\Pi}{\Sigma}{a}$ 
for some types $\Sigma\subseteq\Pi \subseteq \wp A$ and $T_i
\subseteq A$ such 
that $a\notin \bigcup\Sigma$. 	
\label{pt:ofoeifcontinuous}	%
\item 
The formula $\phi$ is functionally continuous in $B \subseteq A$ iff
it is
equivalent to a formula in the basic form $\bigvee 
\mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{\Sigma}{+}$ for some types 
$\Sigma\subseteq \pw A$, $\Psi \subseteq \pw B$ and $T_i \subseteq B$
such that
(1) for all $b \in B$, $b\notin \bigcup\Sigma$ and (2)
$T_1,\dots,T_k$ and each 
$S \in \Psi$ are either empty or singletons. 
\label{pt:ofoeifunctionalcontinuous}	%
\item If $\phi$ is monotone in every element of $A$ (i.e., 
$\phi\in{\ofoei}^+(A)$) then $\phi$ is continuous in $a \in A$ iff it
is
equivalent to a formula in the basic form 
$\bigvee \posdbnfofoei{\vlist{T}}{\Pi}{\Sigma}$ for some types
$\Sigma\subseteq\Pi \subseteq A$ and $T_i \subseteq A$ such that 
$a\notin \bigcup\Sigma$. 
\label{pt:ofoeimonotone}
\end{enumerate}
\end{corollary}

\begin{proof}
	For \ref{pt:ofoeifcontinuous} and \ref{pt:ofoeimonotone}, the
observation is that in order to obtain $\Sigma\subseteq\Pi$ in the
above normal forms it is enough to use
Proposition~\ref{prop:bfofoei-sigmapi} before applying the
translation. For \ref{pt:ofoeifunctionalcontinuous}, fix a model
$(D,V)$ where $\bigvee \mondbnfofoei{\vlist{T}}{\Psi \cup
\Sigma}{\Sigma}{+}$ is true. This means that a certain disjunct
$\mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{ \Sigma}{+}$, by
definition unfolding as
	\begin{equation*}%\label{eq:basicformolque}
	\begin{aligned}
%&\underbrace{\exists \vlist{x}.\Big( \arediff{\vlist{x}} \land\bigwedge_i \tau^+_{T_i}(x_i)\ \land 
%\forall z.(\lnot\arediff{\vlist{x},z} \lor \bigvee_{S\in \Psi \cup
%\Sigma} \tau^+_S(z) \lor \bigvee_{S\in \Sigma}
%\tau^+_S(z)}_{\mondbnfofoe{\vlist{T}}{\Psi \cup \Sigma}{+}}  \\
%& \land \underbrace{\dqu y.\bigvee_{S\in\Sigma} \tau^+_S(y) \Big)
%\land \bigwedge_{S\in\Sigma} \qu y.\tau^+_S(y)}_{\psi},
&\exists \vlist{x}.\Big( \arediff{\vlist{x}} \land \bigwedge_i
\tau^+_{T_i}(x_i)\ \land 
 \forall z.(\lnot\arediff{\vlist{x},z} \lor \!\!\!\bigvee_{S\in \Psi
\cup \Sigma}\!\!\! \tau^+_S(z) 
 \land \dqu y. \!\bigvee_{S\in\Sigma}\! \tau^+_S(y) \Big) \land
\bigwedge_{S\in\Sigma} \qu y.\tau^+_S(y),
\end{aligned}
\end{equation*}
is true. Because by assumption $B \cap \Sigma = \emptyset$, point
\ref{pt:ofoeifcontinuous} yields a restriction $V'$ of $V$ such that
$(D,V') \models \mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{
\Sigma}{+}$ and $V'$ witnesses continuity of $\phi$ in $B$. %For
functionality, observe that $\mondbnfofoei{\vlist{T}}{\Pi}{\Psi \cup
\Sigma}{+}$ is the conjunction of sub-formulas
$\mondbnfofoe{\vlist{T}}{\Psi \cup \Sigma}{+}$ (first line of
\eqref{eq:basicformolque}) and $\psi$ (second line). 

For functionality, the syntactic shape of
$\mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{ \Sigma}{+}$ implies that
$(D,V')$ can be partitioned in three sets $D_1$, $D_2$ and $D_3$ as
follows: $D_1$ contains elements $s_1, \dots, s_k$ witnessing types
$\tau^+_{T_1},\dots, \tau^+_{T_k},$ respectively; among the remaining
elements, there are infinitely many witnessing $\tau^+_S$ for each
$S\in \Sigma$ (these form $D_2$), and finitely many not witnessing
any such $\tau^+_S$ but witnessing $\tau^+_R$ for some $R \in \Psi$
(these form $D_3$). If we now prune any other assignment of
predicates to elements of $D$ but for the types they witness
according to this description, we obtain a restriction $V''$ of $V'$
which still makes $\mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{
\Sigma}{+}$ true. Moreover because $T_1,\dots,T_k$ and each $S \in
\Psi$ are empty or singleton subsets of $B$ and $\Sigma \cap B =
\emptyset$, it shows that $\mondbnfofoei{\vlist{T}}{\Psi \cup
\Sigma}{ \Sigma}{+}$ is functional in $B$, and still witnesses its
continuity because $V'$ does and $V''$ is a restriction of $V'$.
%Then, because $T_1,\dots,T_k,\Psi$ are empty or singletons,
Proposition \ref{lemma:functionalsentenceofoe} yields a restriction
$V''$ of $V'$ such that $(D,V'') \models \mondbnfofoe{\vlist{T}}{\Psi
\cup \Sigma}{+}$ and $V''$ witnesses functionality in $B$ of
$\mondbnfofoe{\vlist{T}}{\Psi \cup \Sigma}{+}$. In order for such
$V''$ to witness continuity in $B$ and make
$\mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{\Sigma}{+}$ true, it must
preserve the condition imposed by $\psi$, i.e. that infinitely many
nodes are marked with each $S \in \Sigma$ and only finitely many are
not marked with any $S \in \Sigma$. It can be checked by inspection
of $\mondbnfofoe{\vlist{T}}{\Pi}{\Psi \cup \Sigma}{+}$ that such a
$V''$ is definable by pruning the valuation $V'$ only for finitely
many elements of $D$. Therefore, $\psi$ remains true, $(D,V'')\models
\mondbnfofoei{\vlist{T}}{\Psi \cup \Sigma}{ \Sigma}{+}$ and thus also
$(D,V'') \models \phi$ as required. 
\end{proof}

\bigskip \hrule \bigskip



==> neutral/ssec-3-af.tex <==
% !TEX root = ../00CFVZ_TOCL.tex
\subsection{Automata to formulas}
   \label{sec:parity-to-mc}

It is well-known that there are effective translations from automata to formulas
and vice versa~\cite{ALG02}.
The results on $\oslang$-automata that we need in this paper are the 
following.

\begin{theorem}\label{t:autofor}
There is an effective procedure that, given an automaton $\bbA$ in 
$\Aut(\oslang)$, returns a formula $\xi_{\bbA} \in \mu\oslang$ which satisfies
the following properties:
\begin{enumerate}[(1)]
    
\item $\xi_{\bbA}$ is equivalent to $\bbA$;

\item $\xi_{\bbA} \in \mu_{D}\oslang$ if $\bbA \in \AutW(\oslang)$;

\item $\xi_{\bbA} \in \mu_{C}\oslang$ if $\bbA \in \AutWC(\oslang)$.
\end{enumerate}
\end{theorem}

\begin{theorem}\label{t:fortoaut}
Let $\oslang$ be a on-step language that is closed under taking conjunctions and 
disjunctions.
Then there is an effective procedure that, given a formula $\xi \in \mu\oslang$
returns an automaton $\bbA_{\xi}$ in $\Aut(\oslang)$, which satisfies the 
following properties:
\begin{enumerate}[(1)]
\item $\bbA_\xi$ is equivalent to $\xi$;
\item  $\bbA_\xi \in \AutW(\oslang)$ if $\xi \in \mu_{D}\oslang$;
\item  $\bbA_\xi \in \AutWC(\oslang)$ if $\xi \in \mu_{C}\oslang$.
\end{enumerate}
\end{theorem}

